Disabling equational theories in unification for cryptographic protocol analysis through tagging

In this paper, we show a new tagging scheme for cryptographic protocol messages. Under this tagging, equational theories of operators such as exclusive-or, binary addition etc. are effectively disabled, when terms are unified. We believe that this result has a significant impact on protocol analysis and security, since unification is at the heart of symbolic protocol analysis. Hence, disabling equational theories in unification implies disabling them altogether in protocol analysis for most operators and theories.

==> proofs.tex <==
\section{Proof of main result - Theorem~\ref{t.main-result}}\label{s.proofs}

\begin{theorem}\label{ta.main-result}

Let $T$ be a set of \dnutsat{} terms. Suppose, $m, t \in T$ where $m, t$ are not variables or sequences. Then, $(m \approx_{(\std \cup \eqth)} t) \Ra (m \approx_{(\std \cup \feqop)} t)$.

\end{theorem}


